Reservoir: Named Data for Pervasive Computation Reuse at the Network Edge

In edge computing use cases (e.g., smart cities), where several users and devices may be in close proximity to each other, computational tasks with similar input data for the same services (e.g., image or video annotation) may be offloaded to the edge. The execution of such tasks often yields the same results (output) and thus duplicate (redundant) computation. Based on this observation, prior work has advocated for "computation reuse", a paradigm where the results of previously executed tasks are stored at the edge and are reused to satisfy incoming tasks with similar input data, instead of executing these incoming tasks from scratch. However, realizing computation reuse in practical edge computing deployments, where services may be offered by multiple (distributed) edge nodes (servers) for scalability and fault tolerance, is still largely unexplored. To tackle this challenge, in this paper, we present Reservoir, a framework to enable pervasive computation reuse at the edge, while imposing marginal overheads on user devices and the operation of the edge network infrastructure. Reservoir takes advantage of Locality Sensitive Hashing (LSH) and runs on top of Named-Data Networking (NDN), extending the NDN architecture for the realization of the computation reuse semantics in the network. Our evaluation demonstrated that Reservoir can reuse computation with up to an almost perfect accuracy, achieving 4.25-21.34x lower task completion times compared to cases without computation reuse.

==> sections/DesignOverview.tex <==
\section{Motivation and Design Overview}
\label{sec:overview}

%In this section, we first motivate \sol and we then present an overview of the \sol design. 

\subsection{Motivation}

To motivate \sol, let us consider a video surveillance use case (Figure~\ref{Figure:re-use}), where cameras capture traffic snapshots in a smart city for traffic management purposes. Such cameras may have snapshot (frame) capture rates ranging from a snapshot every couple of seconds up to several snapshots per second, while they may also rotate to capture snapshots across their full capture width. For example, a camera in Figure~\ref{Figure:re-use} may rotate to estimate the traffic volume for the lanes travelling in the same direction of an intersection, Consecutive camera snapshots, which may be considerably similar, are offloaded to an \EN, so that the number of cars is detected and the traffic volume is estimated. As a result, executing a car detection service on consecutive snapshots (\eg snapshots $n-1$ and $n$) may yield the same execution results. To this end, there is no need to execute the service from scratch for snapshot $n$, but we can rather reuse the results of service execution for snapshot $n-1$ (\ie the previous snapshot).  Even if the camera is stable (does not rotate), with capture rates between a snapshot every couple of seconds and several snapshots per second, it is likely that consecutive snapshots will still be considerably similar. In addition to having an \EN reusing the execution results of previously offloaded snapshots, the camera itself can cache the results of previous snapshots (if its resources allow), so that they are reused locally for consecutive (similar) snapshots, without the need to offload these snapshots at the edge.

In another use case, let us consider a cognitive assistance application, which enables visual search by identifying objects in scenes captured by Augmented Reality (AR) headsets or pictures taken by mobile phones. For example, users exploring a city capture scenes of famous sights with their AR headsets or take pictures of the sights with their mobile phones in order to acquire more information/content about these sights, such as podcasts, videos, information about their history and creators. In this context, %as we illustrate in Figure~\ref{Figure:re-use2}, 
users exploring New York capture scenes or take pictures of the Statue of Liberty (\eg from different angles or distances) and offload these scenes/pictures as the inputs of tasks for a service at the edge, which identifies the sight and returns information/content about it. These input scenes/pictures are similar, thus yielding the same execution results.

In both previous use cases, a massive number of devices may offload large numbers of similar tasks at the edge. For example, certain cities in China are estimated to have up to 2.5M CCTV cameras each~\cite{cctv-countries}, while major cities in Europe and the US are also estimated to have several tens or even hundreds of thousands of CCTV cameras~\cite{cctv-countries, cctv-london}. In addition, popular sights around the world attract several millions of visitors annually and up to tens of thousands of visitors daily. For example, the Statue of Liberty attracts about 4.5M visitors annually and about 10K visitors daily~\cite{liberty}, while the Louvre museum attracts 10M visitors annually and about 15K visitors per day, containing more than 380K objects and displaying 35K works of art~\cite{louvre}. Such use cases may result in the execution of massive amounts of duplicate (redundant) computation, since offloaded tasks may include similar inputs. To this end, computation reuse can result in: (i) eliminating the execution of duplicate computation; (ii) reducing the execution times of tasks; and (iii) reducing the usage of computing resources at the edge and ensuring their effective utilization. 

\noindent \textbf{Why do we realize \sol over NDN:} NDN offers a communication model that makes the network directly aware of the communication context, since each packet carries a semantically meaningful name. \sol builds on top of and extends NDN naming and name-based forwarding combined with LSH in order to: (i) make the network directly aware of the semantics of computation reuse; (ii) enable the identification of similar tasks in the network in a light-weight manner; and (iii) enable the forwarding of tasks in a \enquote{computation reuse aware} fashion with nominal performance overhead, so that similar tasks are forwarded towards the same \ENs and the reuse of computation is facilitated.

\begin{figure}[!t]
%\vspace{-0.2cm}
 \centering
 \includegraphics[width=0.9\columnwidth]{figs/Reuse-crop.pdf}
 \vspace{-0.5cm}
 \caption{A video surveillance use case, where traffic snapshots are captured in a smart city for traffic management purposes. Consecutive snapshots are offloaded as the inputs of tasks that invoke a car detection service at the edge. The captured snapshots are likely to yield the same execution results due to considerable similarity among them.}
 \label{Figure:re-use}
 \vspace{-0.5cm}
\end{figure}

%\begin{figure}[!t]
%\vspace{-0.1cm}
% \centering
% \includegraphics[width=0.8\columnwidth]{figs/Use-case-crop.pdf}
% \vspace{-0.2cm}
% \caption{Users capture scenes with their AR headsets or take pictures with their mobile phones of the Statue of Liberty from different angles/distances to acquire information/content (\eg podcasts, videos) about it. The pictures are offloaded as the inputs of tasks to an edge service, which recognizes the sight and returns information about it. The scenes/pictures are similar (depict the same sight from different angles or distances) and yield the same execution results (information about the Statue of Liberty).}
% \label{Figure:re-use2}
% \vspace{-0.5cm}
%\end{figure}

\subsection{Design Assumptions, Overview, and Goals}
\label{subsec:overview}

We assume the existence of edge networks (\enquote{cloudlets})~\cite{satyanarayanan2009case}, which consist of \ENs and NDN forwarders. The \ENs are server-class nodes with computing and storage resources, and offer a set of services (\eg object recognition, face detection) to users. \ENs may either be a single hop (\eg directly attached to LTE/5G base stations) or a few hops away from users (\eg at the edge of the core network). Users offload tasks, which are forwarded by NDN forwarders towards the \ENs of an edge network. Each task invokes one of the offered services, while it may also carry input data to be passed to the invoked service for its execution (\eg an object detection service may expect an image as input data). Each \EN and user device have a name prefix, which is used for direct communication with this specific \EN or device.

The workflow of the \sol operation is illustrated in Figure~\ref{Figure:workflow}. In \sol, a task is represented as a request (Interest) that identifies the service to be invoked in its name. First, users apply locality sensitive hash functions to the input data of a task and attach the resulting hash to the name of the Interest\footnote{We discuss approaches for users to discover the locality sensitive hash function(s) that they need to apply to the task input data in Section~\ref{sec:discussion}.}. As a result, tasks that invoke the same service with similar inputs are likely to have identical names, thus being able to: (i) reuse results of similar previously executed tasks that might be cached in the CS of NDN forwarders;
%or user devices 
and (ii) get aggregated in the network 
if a similar task is currently pending in the PIT of NDN forwarders. %or user devices. 
Each user device also runs a local NDN forwarder instance, thus it can cache the results of previously executed tasks for reuse in its local CS and aggregate subsequent similar tasks in its local PIT depending on the availability of its local resources.
If (i) and (ii) are not possible, offloaded tasks will be forwarded towards \ENs by NDN forwarders in a \enquote{computation-reuse aware} manner, so that similar tasks are forwarded towards the same \EN in order to facilitate the reuse of the execution results among similar tasks. To make NDN forwarders aware of the semantics of computation reuse, we extend their Interest forwarding pipeline by introducing a reuse FIB (rFIB) data structure (Figure~\ref{Figure:forwarding}), which stores reuse-related information in the network. Finally, once a task $t_{new}$ is received by an \EN, LSH will enable the \EN to effectively search for a previously executed task $t_{previous}$ of the same service, so that the similarity between the input data of $t_{new}$ and $t_{previous}$ exceeds a certain similarity threshold. If such a task $t_{previous}$ is found, the \EN will reuse the results of $t_{previous}$, otherwise, the \EN will execute $t_{new}$ from scratch.

The \textbf{goal} of the \sol design is not only to facilitate the reuse of computation at the network edge, but also to: 

\begin{itemize}[wide, labelwidth=!, labelindent=0pt]

\item \textbf{Impose nominal performance overhead on user devices} for receiving the benefits of computation reuse.

\item \textbf{Impose nominal performance overhead on the NDN network} for the identification and forwarding of similar tasks in a reuse aware manner.

\item \textbf{Enable \ENs to find} the execution results of previously executed similar tasks \textbf{as quickly as possible.}

\end{itemize}

\begin{figure}[t]
%\vspace{-0.1cm}
 \centering
 \includegraphics[width=1\columnwidth]{figs/sol WorkFlow-crop.pdf}
 \vspace{-0.5cm}
 \caption{Workflow of the \sol operation.}
 \label{Figure:workflow}
 \vspace{-0.7cm}
\end{figure}

%\subsection{Design Overview}



==> sections/Discussion.tex <==
\section{Discussion}
\label{sec:discussion}

In this section, we discuss considerations and extensions of the \sol design. %, which we plan to explore in the future.

%\subsection{User Onboarding and Discovery of LSH functions}
%\label{subsec:discovery}

% cite the discovery from ICedge and say that we can use similar mechanisms to discover LSH functions

\noindent \textbf{User onboarding and discovery of locality sensitive hash functions:} Before users can start offloading tasks at the edge, they may need to onboard an edge network, as well as discover the offered services and the available computing resources. Due to mobility, users may also onboard different edge networks over time (\eg while moving from one part of a city to another). To achieve that, NDN-based mechanisms have been proposed~\cite{mastorakis2019towards}, which enable users to onboard an edge network by communicating with the closest \EN. Such mechanisms can be used in \sol as well. During the onboarding process, users can discover the family of locality sensitive hash functions to be used and pass custom functions (\eg in the form of lambda functions~\cite{fischer1972lambda}) to \ENs for future execution, if needed.

% Tasks with minor input data similarities

\noindent \textbf{Tasks with minor similarities between their input data:} As we mentioned in Section~\ref{sec:overview}, not all use cases/applications may involve tasks with input data, which exhibits temporal, spatial, and semantic similarities. \sol can be extended to accommodate such cases. An option could be that application developers indicate whether they expect their applications to involve tasks with similar input data. Another option could be for \ENs to identify applications that do not offload tasks with similar time over time and inform users during the onboarding process mentioned above. Both options allow for the identification of applications that exhibit minor input data similarities, enabling such applications to indicate to the edge network infrastructure that their tasks should not be treated in the context of computation reuse (\eg by creating and offloading tasks with a special component in their names or a dedicated flag in their packet format). This enables: (i) applications to eliminate the overhead associated with generating a locality sensitive hash for each task, thus generating a less expensive hash instead (\eg CRC32, SHA1), which will be used as the third name component of a task's name (following the namespace design of Section~\ref{subsec:namespace}); (ii) the edge network infrastructure to eliminate the overhead of performing \enquote{computation-reuse aware} task forwarding based on the rFIB, but rather forward tasks based on the FIB directly; and (iii) \ENs to eliminate the overhead associated with nearest neighbor searches. The same mechanism can also apply to applications where tasks with similar input data may yield substantially different execution results. 

%\subsection {Populating the rFIBs of NDN Forwarders}
%\label{subsec:populate}

\noindent \textbf{Populating the rFIBs of NDN forwarders:} In Section~\ref{sec:design}, we presented the structure of rFIB and how rFIB is used to make the network aware of the semantics of computation reuse. However, the rFIB of each NDN forwarder needs to be populated with entries. rFIBs can be populated in different ways: (i) through NDN-based routing protocols~\cite{hoque2013nlsr, ghasemi2018muca}; or (ii) by integrating a Software-Defined Networking (SDN) control plane with \sol~\cite{zuraniewski2017facilitating}. Specifically, NDN-based routing protocols can be extended to propagate information about the computation reuse semantics from the \ENs to the NDN network. %and install them on NDN forwarders.
Alternatively, each edge network may have a (logically) centralized SDN control plane, which collects information from \ENs and NDN forwarders over time and installs rFIB entries on NDN forwarders.

%Given the potentially small scales of edge networks and the dynamic conditions at the edge (\eg fast changing rates of user requests, usage of computing resources), an SDN control plane and its (logically) centralized network intelligence may enable NDN forwarders to adapt to conditions at the edge by collecting information from \ENs and populating the forwarders' rFIBs accordingly. 

% Incorporate such information onto a routing protocol, use self-learning, or an SDN controller

%\subsection {Balancing the Load Among \ENs}

\noindent \textbf{Assigning LSH buckets and balancing the load among \ENs:} In \sol, each \EN is responsible for a range of LSH buckets per hash table for a service. To this end, \ENs either need a distributed mechanism to coordinate and assign LSH buckets among themselves or LSH buckets can be assigned to \ENs through a central entity (\eg an SDN controller as we previously discussed). However, this does not ensure that the load will be evenly distributed among \ENs, since the input data of offloaded tasks may unevenly index the buckets assigned to the available \ENs. As a result, certain \ENs may become more loaded than others, since they will execute more tasks over time. In such cases, the dynamic reassignment of buckets may be needed, aiming to: (i) evenly distribute the load among \ENs; and (ii) maintain the assignment of consecutive blocks of buckets to \ENs, since similar data is likely to be hashed in adjacent, if not the same, buckets of a hash table~\cite{lv2007multi}. Such reassignment operations %may take place through the same mechanism as the initial assignment of buckets, while reassignment operations 
may also need to be followed by updates of the rFIB entries of NDN forwarders. %in the edge network.

\noindent \textbf{Deploying \sol over IP-based edge network infrastructure:} Running on top of NDN, \sol can be also deployed on top of an IP-based edge network infrastructure by running NDN as an overlay on top of TCP/IP or UDP/IP (as we did for our experimental evaluation in Section~\ref{subsec:realworld}). In such cases, NDN forwarders can be installed on user devices and \ENs, and can also be deployed on edge routers to enable NDN communication over existing IP-based infrastructures.

% Talk about bucket re-distribution among ENs

%\subsection {Task Offloading to \ENs at Different Distances from Users}

% \subsection{Privacy Considerations}

% Talk about ENs that might offer different network latency to users. Say that we could have an objective function that considers RTT to ENs plus computation reuse

%\subsection {Reuse Among Services of the Same Nature}

% Say that reuse of possible among services of the same nature (e.g., objection detection through different algorithms), not only strictly for the same service

%\subsection {Storage Optimization at \ENs}

%\noindent \textbf{LSH variants and optimizations:} As discussed in Section~\ref{sec:eval}, for the implementation of \sol, we made use of the FALCONN library~\cite{andoni2015practical} to realize LSH and perform similarity searches at \ENs, achieving satisfactory accuracy and performance for image data as the input of offloaded tasks. LSH variants and optimizations have been proposed for different types of data (\eg images, speech, text)~\cite{guo2018foggycache, sundaram2013streaming}. To this end, different LSH variants can be selected depending on the use case and the expected type of task input data.

\noindent \textbf{Storage optimization at \ENs:} The \sol design can be complemented with mechanisms for storage optimization at \ENs. Such optimizations may span a wide spectrum of solutions, such as distributed file systems~\cite{shvachko2010hadoop}, database designs (\eg relational, object-oriented, graph-based)~\cite{angles2008survey}, key-value stores~\cite{jin2017netcache}, or even eviction policies for the replacement of stored tasks with newly executed tasks~\cite{guo2018potluck, drolia2017cachier}. Such mechanisms can help the task storage operations at \ENs scale and further reduce the time needed for \ENs to find and reuse the results of previously executed similar tasks. Furthermore, services of the same nature (\eg object detection services that are implemented through different algorithms) may share the same hash tables to further reduce the number of tables that need to be maintained by \ENs, since such services are expected to offer the same overall functionality (\eg object detection).

% Talk about storage optimization at ENs and eviction (replacement) of previously executed tasks that have been stored.

